SoccerNet Game State Reconstruction: End-to-End Athlete Tracking and Identification on a Minimap

Tracking and identifying athletes on the pitch holds a central role in collecting essential insights from the game, such as estimating the total distance covered by players or understanding team tactics. This tracking and identification process is crucial for reconstructing the game state, defined by the athletes' positions and identities on a 2D top-view of the pitch, (i.e. a minimap). However, reconstructing the game state from videos captured by a single camera is challenging. It requires understanding the position of the athletes and the viewpoint of the camera to localize and identify players within the field. In this work, we formalize the task of Game State Reconstruction and introduce SoccerNet-GSR, a novel Game State Reconstruction dataset focusing on football videos. SoccerNet-GSR is composed of 200 video sequences of 30 seconds, annotated with 9.37 million line points for pitch localization and camera calibration, as well as over 2.36 million athlete positions on the pitch with their respective role, team, and jersey number. Furthermore, we introduce GS-HOTA, a novel metric to evaluate game state reconstruction methods. Finally, we propose and release an end-to-end baseline for game state reconstruction, bootstrapping the research on this task. Our experiments show that GSR is a challenging novel task, which opens the field for future research. Our dataset and codebase are publicly available at https://github.com/SoccerNet/sn-gamestate.

==> sections/Y_ignored.tex <==
\section{Introduction}
\label{sec:intro}
% Keywords that should appear: holy grail, minimap, radar view

% \textbf{What is game state reconstruction}, it can be seen as a compression task to turn raw pixel level information into high-level and highly-compressed semantic information about the game. 
% Thanks to the game state reconstruction data, one can build a minimap/radar view of the game, as illustrated in Fig X.
% Show pull figure with video + minimap.

% \textbf{Why is it needed}: Sports analytics and personalized content, coaching, scouting, etc. Game State Reconstruction = Holy Grail task for high-level video understanding in sports.

% \textbf{What currently exists}: no open source dataset or codebase, proprietary software. Because annotation cost expensive, software complex, great value for the sport industry and companies need to keep competitive advantage. No end-to-end metric either. 

% \textbf{How we solve that}: new task, dataset, baseline and evaluation metric to foster further research on this domain. 

% \textbf{Contributions} = novel annotations, novel task definition, novel evaluation metric, first open-source end-to-end solution for this task.

% Text from the Github/Website:

% The SoccerNet Game State Recognition task is a novel high-level computer vision task that is specific to sports analytics. It aims at recognizing the state of a sport game, i.e., identifying and localizing all sports individuals (players, referees, ..) on the field based on a raw input videos
% SoccerNet GS (Game State) takes raw broadcast videos as input and outputs the position of all individuals on the court, their role (player, goalkeeper, referee, ...), team and their jersey number. The output of the game state task can therefore be used to display a minimap or radar view of the game, as illustrated in the image.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\textit{(first raw draft, to be improved with several iterations)}
Recently, sports companies and teams have shown growing interests in collecting athlete-centric data. 
%One major focus is centered on tracking and identifying players on the sports pitch throughout an entire game from available videos, since this information holds immense value.
One key focus area lies in tracking and identifying athletes on the sports field throughout the entire game, using available video footage. %, given the immense value this information holds.
Indeed, such data holds immense value for a broad spectrum of sports analytics tools, ranging from helping coaches in improving their team performance or assisting scouters in discovering new talents, to offering valuable insights for bookmakers, doctors, and physiotherapists, and enabling the creation of personalized content to boost fan engagement~\cite{Chen2010Personalized,  Chen2011Automatic, Fernández2010Browsing}.


%However, manually generating such data through human annotators is time-consuming and therefore expensive. 
However, the manual generation of such data through human annotators is a time-consuming process, making it inherently expensive.
Sensor-based solutions offer a time-efficient alternative, but require athletes to wear special, sometimes expensive, equipment. 
Recently, automatic solutions based on optical tracking systems have gained prominence. These systems necessitate the installation of sophisticated, well-calibrated static multi-camera setups in stadiums. Hence, they come with significant drawbacks in terms of cost and scalability, which restricts their use to elite competitions, exemplified by their deployment at events like the 2022 Qatar World Cup.
%the installation of sophisticated multi-camera systems in stadiums are expensive and lack scalability.
Recent advancements in computer vision and deep learning opened up a growing potential to automatically and reliably extract athlete localization and identification data solely from the feeds captured by broadcast moving cameras.
%
%With recent advancements in computer vision and deep learning, there is a growing potential to automatically and reliably extract the player localization and identification data using just the video feeds from broadcast cameras.
% Having access to reliable technology based on computer vision to extract such information could significantly change the sports industry, offering a scalable and cost-effective solution that can be widely adopted to improve various aspects of sports.

\input{figures/pull_figure}

%Despite its importance for the sports sector, there exists no proper formalism for this automated generation of player localization and identification data.
%Existing solutions and datasets are often locked within the proprietary software of sports companies, inaccessible to researchers given the high annotation and development cost, and the need for these companies to keep their competitive advantage.
%Moreover, the absence of standardized benchmarks and evaluation metrics further impedes research in this area.

%To fill this gap, we believe there are three key initiatives to be dealt with: 1) providing a publicly available dataset, 2) releasing an open-source framework as the starting point for the community, and 3) introducing a novel metric specialized for this task.

In this work, we therefore introduce the novel concept of \emph{game state} for sports and propose a novel \textbf{G}ame \textbf{S}tate \textbf{R}econstruction (\textbf{GSR}) task and dataset to support research.% that aims to touch the three mentioned key initiatives.
The game state refers to the precise and comprehensive representation of all athlete positions and identities on a 2D top-view, or minimap, of the pitch at any given moment during a sports match, providing an accurate condensed information of the ongoing gameplay dynamics.
Therefore, given raw broadcast videos as input, the game state reconstruction task aims at accurately tracking and identifying all individuals involved in a sports game on a minimap of the pitch as illustrated in Figure~\ref{fig:pull_figure}.
To support research in the field, we publicly release \emph{SoccerNet-GSR}, the first dataset for game state reconstruction, comprising $200$ $30$-second clips fully annotated with all athlete positions on the 2D image and real-world pitch coordinate systems, and their identification information, including their role, team, and jersey number. Our annotations also include tracking data of all pitch lines to support the development of video camera calibration methods.
Furthermore, we propose the first end-to-end baseline, providing a first modular solution for game state reconstruction, based on state-of-the-art tracking, re-identification, team affiliation, jersey number recognition, and camera calibration methods.
Finally, we introduce a novel metric, \emph{GS-HOTA}, to evaluate and benchmark future research on our game state reconstruction task. 
Our analysis shows the challenging nature of game state reconstruction and emphasizes that the introduction of this new task, dataset, and baseline establishes an ideal platform for future research in the field, aiming to democratize access to this valuable data for all leagues.
%In other words, this entails pinpointing each person's position within the pitch's coordinate system and providing comprehensive details to distinguish them.
%More precisely, this involves localizing each person's position within the pitch's coordinate system while predicting various sports-related attributes, such as their roles, team affiliations, and jersey numbers, thereby achieving a unique identification.
%Ultimately, the extracted Game State information enables the generation of comprehensive visualizations, such as minimaps or radar views of the so, offering valuable insights into the game dynamics, as depicted in \cref{fig:pull_figure}.
%GSR can be therefore interpreted as a compression task to turn raw pixel information from videos into high-level and highly-compressed semantic information about the game. 
%In essence, game state reconstruction represents the holy grail of multi-object tracking in the realm of teamsports competitions.

\mysection{Contributions. } We summarize our contributions as follows. 
\textbf{(i)} We define the new concept of \emph{game state} and propose a novel \emph{Game State Reconstruction} task aiming to track and identify all athletes on a minimap of the pitch.
\textbf{(ii)} We publicly release the \textbf{SoccerNet-GSR} dataset, the first open-source sports video dataset that includes athlete tracking and identification data in the pitch coordinate system.
\textbf{(iii)} We propose a first end-to-end baseline for game state reconstruction in football videos.
\textbf{(iv)} We introduce \textbf{GSR-HOTA}, a new evaluation metric to evaluate and benchmark game state reconstruction methods.%, thereby offering an effective benchmarking metric for this task.

%Finally, we conduct thorough experiments to validate our baseline and metric.
%Our findings reveal the complexity of this task and demonstrate that further research efforts are necessary to enhance the overall GSR performance, both in terms of evaluation metrics and inference speed. 

% Through our work, we aim to foster further research on this challenging topic, by offering a robust framework for researchers to benchmark their methods

% %%%%%%%


==> tables/inference_time.tex <==
\begin{table}[]
    \centering
\caption{
Timing analysis of the GSR-Baseline modules.
}
\label{table:baseline-timing}
\begin{tabular}{l|rr}% \toprule
Module             & Batch Size & Avg. FPS $\uparrow$ \\ \midrule
Yolov8          & 32 & 16.5   \\
PRTReID         & 16 & 14.5   \\
StrongSORT         & N/A& 45.2   \\
TVCalib Segm.   & 16 & 2.9    \\
TVCalib Calib.  & 512& 7.6    \\
MMOCR           & 32 & 3.8    \\ \midrule
Total           & N/A& 1.1    \\
\end{tabular}
\end{table}
